Measuring Technological Complexity Using Japanese Patents

As international competition intensifies in technologies, nations need to identify key technologies to foster innovation. However, the identification is challenging due to the independent and inherently complex nature of technologies. Traditionally, analyses of technological portfolios have been limited to simple evaluations, indicating merely whether a technology is specialized. We propose evaluating TCI at the corporate level, which provides finer granularity and more detailed insights than conventional regional evaluations by using Japanese patent data spanning fiscal years 1981 to 2010. Specifically, we analyze a bipartite network composed of 1,939 corporations connected to technological fields categorized into either 35 or 124 classifications. Our findings quantitatively characterize the ubiquity and sophistication of each technological field, reveal detailed technological trends reflecting broader societal contexts, and demonstrate methodological stability even when employing finer technological classifications. Additionally, our corporate-level analysis allows consistent comparisons across different regions and technological fields, clarifying regional advantages in specific technologies. The corporate level analysis also reveals a new possibility for formulating an innovation strategy.

==> diffreamble.tex <==
% 色と取り消し線の見た目を指定（新=赤、旧=黒取り消し線）
\RequirePackage[normalem]{ulem}
\RequirePackage{xcolor}
\providecommand{\DIFadd}[1]{\textcolor{red}{#1}}
\providecommand{\DIFdel}[1]{\textcolor{black}{\sout{#1}}}
\providecommand{\DIFaddbegin}{\color{red}}
\providecommand{\DIFaddend}{\color{black}}
\providecommand{\DIFdelbegin}{\color{black}\begingroup
  \markoverwith{\textcolor{black}{\rule[.5ex]{2pt}{1pt}}}\ULon}
\providecommand{\DIFdelend}{\ULoff\endgroup}

